Explainable Data Imputation using Constraints

Data values in a dataset can be missing or anomalous due to mishandling or human error. Analysing data with missing values can create bias and affect the inferences. Several analysis methods, such as principle components analysis or singular value decomposition, require complete data. Many approaches impute numeric data and some do not consider dependency of attributes on other attributes, while some require human intervention and domain knowledge. We present a new algorithm for data imputation based on different data type values and their association constraints in data, which are not handled currently by any system. We show experimental results using different metrics comparing our algorithm with state of the art imputation techniques. Our algorithm not only imputes the missing values but also generates human readable explanations describing the significance of attributes used for every imputation.

==> implementation.tex <==
\section{Implementation}

==> res.tex <==


\begin{figure*}
\centering
\subcaptionbox{Polynomials}{\includegraphics[width=0.30\textwidth]{figures/polynomial_V1}}%
\subcaptionbox{Iris}{\includegraphics[width=0.30\textwidth]{figures/sklearn_iris_V1}}%
\subcaptionbox{Ecoli}{\includegraphics[width=0.30\textwidth]{figures/ecoli_V1}}%
\par
\subcaptionbox{Breast Cancer}{\includegraphics[width=0.30\textwidth]{figures/breast_cancer_V1}}%
\subcaptionbox{Wine}{\includegraphics[width=0.30\textwidth]{figures/wine_V1}}%
\subcaptionbox{Diabetes}{\includegraphics[width=0.30\textwidth]{figures/diabetes}}%
\caption{Numerical Imputation results on various datasets.}
\label{fig:num_results}
\end{figure*}
%\subsection{Categorical Imputation}

\begin{figure*}
\centering
\subcaptionbox{Iris}{\includegraphics[width=0.30\textwidth]{figures/iris_species}}%
\subcaptionbox{Bank Market(Job)}{\includegraphics[width=0.30\textwidth]{figures/bank_ajme_small_job}}%
\par
\subcaptionbox{Bank Market(Marital)}{\includegraphics[width=0.30\textwidth]{figures/bank_ajme_small_marital}}%
\subcaptionbox{Bank Market(education)}{\includegraphics[width=0.30\textwidth]{figures/bank_ajme_small_education}}%
\caption{Categorical Imputation results on various datasets.}
%\label{fig:cat_results}
\end{figure*}
\textbf{Metric.} The normalized root mean square error for a numerical column $c$ with a standard deviation $\sigma_c$, denoted $NRMSE_c$, is computed as follows: 

\[
NRMSE_c = \frac{RMSE_c}{\sigma_c}
\]

The normalized root mean square for a dataset, with $NCOL$ as the set of all numerical columns, is the mean of normalized root mean square error for all numerical columns.
\[
NRMSE = \frac{\displaystyle\sum_c^{NCOL}{NRMSE_c}}{|NCOL|} 
\]



In Figure~\ref{fig:num_results} 
we compare our results with three methods from the fancyimpute package (mean, KNN and matrix factorization) and two methods from the IterativeImputer of sklearn with the estimators RandomForestRegressor and LinearRegression, which are similar to the MissForest approach~\cite{missforest-bioinformatics12,van2018flexible} , and MICE with a linear model~\cite{little2002statistical}; iterative 
imputation here means that 10 consecutive imputation rounds were performed for replacing the missing values in the input columns. All methods were evaluated on one synthetic linear and one synthetic non-linear problem and five real data sets available in sklearn. 
Values were discarded completely at random. In Figure~\ref{fig:num_results} the average root mean-squared error is shown, normalized to the standard deviation for each column.
\textbf{(From Datawig paper) - Values were discarded either completely at random, at random (conditioned on values in another randomly chosen column being in a random interval) or not at random (conditioned on values to be discarded). In Figure~\ref{fig:num_results} the relative mean-squared error is shown, normalized to the highest MSE in a given condition.}

% \textbf{When comparing with mode imputation and datawig, we achieves a median F1-score of $60\%$ across three tasks, imputation of the Wikipedia attributes birth-place, genre and location, with a simple $n$-gram model. Mode imputation reached a median F1-score of $0.7\%$ and string matching $7.5\%$ .}
